Change the Product, Keep the Parameters: Associative Algebra Layers for Transformers

Fast matrix multiplication algorithms keep the product fixed and search for a cheaper way to evaluate it. We instead ask whether a Transformer's learned projections can use a different, cheaper product altogether. Building on an associative-algebra construction that replaces ordinary matrix multiplication with a sparser interaction table over the same weight blocks, we construct a family with quadratic arithmetic in the matrix dimension when the physical block size remains fixed, and derive finite-shape constraints for GPU execution. The construction is provably optimal for its bilinear rank by the Alder--Strassen bound and can be realized as row-typed rectangular projections compatible with causal masking and KV-cached decoding. We provide an empirical test of this approach by training two approximately 110M-parameter decoder-only Transformer LMs from the same recipe and 12.3B-token budget, differing only in their feed-forward layer: one uses ordinary dense matrix multiplication and the other uses the associative-algebra product. Across four prompt domains, the algebraic model achieves a 6.2--7.8\% increase in end-to-end generation throughput, while obtaining lower scores on all three reported downstream metrics. We treat these results as a feasibility and trainability check for the proposed approach at small scale, leaving further investigation to future work.

==> sections/06_expressivity.tex <==
\section{Expressivity}
\label{sec:expressivity}

The arithmetic saving has a precise structural price.  A type-$i$ token sees a star-shaped operator: output group $j$ depends only on input groups $\{i,j\}$.  The full bank contains $d_{\rm in}d_{\rm out}$ independent scalars, and every parameter affects some token type, while a single type realizes a strict star-shaped subspace of dense maps.  For $q\ge2$ and equal square groups, choosing each diagonal block invertible makes this operator invertible.  The restriction therefore removes interactions while preserving possible full rank.

Associativity closes compatible linear layers under the same law.
Pointwise nonlinearities separate successive projections while preserving
their feature dependencies; attention couples the token positions.
The tensor-square law permits additional interactions described in
\cref{app:tensor-square}, but still restricts the layer's function class.
Matching stored parameters therefore allows a change in expressive capacity.
The experiment below measures the resulting quality--throughput trade-off.


==> sections/12_impact_statement.tex <==
\section*{Impact Statement}

This work studies arithmetic reductions in Transformer layers. The pilot
shows higher generation throughput on one GPU with lower downstream scores.
Energy savings require direct measurement. Models using these layers retain
the broader risks of language models, including biased outputs and misuse.
The training corpus combines public instruction and code datasets; future
releases should document licenses, preprocessing, and evaluation overlap.

